Warm-Inflation: a software for first-principles integration of warm inflation power spectra

As part of a PhD thesis entitled `Scalar perturbations in warm inflation and during reheating' we present a software for computing warm inflation observables. In particular, our Mathematica implementation computes the power spectrum, spectral tilt, and tensor-to-scalar ratio for a given momentum scale. Compared with other implementations, we start in a Bunch-Davies state deep inside the horizon, ideally at a time when thermal noise is exponentially suppressed. We integrate gauge-invariant equations for three curvature perturbations across horizon exit. We continue deep enough outside of horizon so that all curvature perturbations agree. Results are illustrated for Standard Model embedded warm inflation, and we also provide notebooks for several other popular potentials and friction coefficients. The theoretical foundations for the code can be found in the main part of the thesis or in earlier papers [1,2]. Specifically, part II derives gauge-invariant, model-agnostic evolution equations, as well as the noise autocorrelator interpolating between quantum and classical domains. Part III presents the general ideas behind the numerical implementation, while part IV presents selected results. The code is described, line-by-line, in Appendix A. The published PhD thesis is available at https://doi.org/10.48620/101166 while the notebooks can be downloaded from https://github.com/alicarogeljblackhole/Warm-Inflation.

==> Chapters/Introduction/figureintro.tex <==



